ENCODE: Encoding NetFlows for Network Anomaly Detection

NetFlow data is a popular network log format used by many network analysts and researchers. The advantages of using NetFlow over deep packet inspection are that it is easier to collect and process, and it is less privacy intrusive. Many works have used machine learning to detect network attacks using NetFlow data. The first step for these machine learning pipelines is to pre-process the data before it is given to the machine learning algorithm. Many approaches exist to pre-process NetFlow data; however, these simply apply existing methods to the data, not considering the specific properties of network data. We argue that for data originating from software systems, such as NetFlow or software logs, similarities in frequency and contexts of feature values are more important than similarities in the value itself. In this work, we propose an encoding algorithm that directly takes the frequency and the context of the feature values into account when the data is being processed. Different types of network behaviours can be clustered using this encoding, thus aiding the process of detecting anomalies within the network. We train several machine learning models for anomaly detection using the data that has been encoded with our encoding algorithm. We evaluate the effectiveness of our encoding on a new dataset that we created for network attacks on Kubernetes clusters and two well-known public NetFlow datasets. We empirically demonstrate that the machine learning models benefit from using our encoding for anomaly detection.

==> sec_methodology.tex <==
\section{Frequency-based Network Anomaly Detection Method}\label{sec:frequency_ad}

==> sec_potential_harm.tex <==
\section{Potential Harm}\label{sect-potential_harm}
For this work, there is potential harm that could stem from publishing this work; one of the datasets that we have used (the ANONYMISED dataset) to evaluate our encoding is generated with the help of real-life participants. IP addresses are collected in the NetFlow data and these are considered to be personally identifiable information. The IP addresses can be used to trace back who participated in the data collection campaign that we have organised. To resolve this issue, we have anonymised the IP addresses before the dataset is publicly released. 

Additionally, we use Elasticsearch to collect NetFlow within our Kubernetes testbed and we have configured it to only collect network traffic that occurs only between the pods that were deployed within the cluster (IP addresses of the participants are therefore not collected). In the case that an attacker manages to de-anonymise the IP addresses in our dataset, the attacker would only get their hands on the internal IP addresses that were used by the pods. These internal IP addresses also reset each time we rebuild the cluster for a new data collection campaign. An attacker would therefore not be able to link an IP address back to a participant that took part in our data collection campaign. 

Furthermore, our data collection campaign was assessed and approved by an ethical committee before it took place. During the assessment, the ethical committee reviewed the potential risks that are associated with our campaign and our plan to mitigate these potential risks.

==> sec_preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}
